Smooth Bilevel Programming for Sparse Regularization

Iteratively reweighted least square (IRLS) is a popular approach to solve sparsity-enforcing regression problems in machine learning. State of the art approaches are more efficient but typically rely on specific coordinate pruning schemes. In this work, we show how a surprisingly simple reparametrization of IRLS, coupled with a bilevel resolution (instead of an alternating scheme) is able to achieve top performances on a wide range of sparsity (such as Lasso, group Lasso and trace norm regularizations), regularization strength (including hard constraints), and design matrices (ranging from correlated designs to differential operators). Similarly to IRLS, our method only involves linear systems resolutions, but in sharp contrast, corresponds to the minimization of a smooth function. Despite being non-convex, we show that there is no spurious minima and that saddle points are "ridable", so that there always exists a descent direction. We thus advocate for the use of a BFGS quasi-Newton solver, which makes our approach simple, robust and efficient. We perform a numerical benchmark of the convergence speed of our algorithm against state of the art solvers for Lasso, group Lasso, trace norm and linearly constrained problems. These results highlight the versatility of our approach, removing the need to use different solvers depending on the specificity of the ML problem under study.

==> sections/old.tex <==
% !TEX root = ../NonCvxReparam.tex

\section{Remarks}


\subsection{A more general formulation?}
Given
\begin{equation}
\min_{\beta,\eta}\frac12 \norm{X \beta -y}_2^2 + \sum \frac{\beta_i^2}{\eta_i} + \Psi(\eta) \quad s.t. \quad \eta\geq 0
\end{equation}
we can apply nonconvex splitting to obtain
\begin{equation} 
\min_{\beta= u\odot v}\frac12 \norm{X u\odot v -y}_2^2 + \norm{u}^2 + \Psi(v\odot v) 
\end{equation}
Then, we see that for each $v$, the optimal  $u$  is of closed form  as a solution to a least squares problem (actually, if the loss function is Lipschitz smooth then its dual is strongly convex, we can write an inner problem which has a unique solution, but the issue is that this is not of closed form). The main idea of this paper is to obtain an unconstrained smooth problem in the variable $v$ so we can apply BFGS -- so we want $v\mapsto \Psi(v\odot v)$ to be differentiable. However, note that the derivative of this is $v \odot \partial \Psi(v\odot v)$, so would this be unique under some partial smoothness condition? In particular, $\partial \Psi(v\odot v)$ is unique when restricted to the model space of $v$?



\subsection{Interpretation as infimal convolution}
 Not sure if this comment is useful, but our nonconvex splitting is a bit like taking an infimal convolution with the quadratic function:
Consider a regulariser of the form
$$
R(w) = \min_{\eta\geq 0} \frac12 \sum_i \eta_i \norm{w_i}^2 + \Psi(1/\eta_i).
$$
The case $\Psi(v) =\frac12 t$ corresponds to the $\ell_1$ norm. What we're doing is
$$
R(w) = \min_{u\odot v = w} \frac12 \norm{u}^2 + \Psi(v\odot v)
$$
This is sort of like an infimal convolution after taking $\log$ and $\exp$, since  $\log(w) = \log(u)+\log(v)$.
That is, writing $\phi = \log(\abs{w})$, we have $R(w) = R(\abs{w}) = \tilde R(\phi)$ where
$$
\tilde R(\phi) = \min_{\mu+\nu = \phi} \frac12 \norm{\exp(\mu)}^2 + \Psi(\exp(2\nu))
$$


\subsection{Interior Point methods and the $\eta$-trick}
\paragraph{Interior point methods}
An example of an interior point method applied to the Lasso is \cite{koh2007interior}. The idea is to rewrite 
$$
\min_{\beta} \norm{\beta}_1 + \frac12 \norm{X\beta - y}_2^2
$$
as
\begin{align*}
\min_{\beta,u} &\sum_i u_i + \frac12 \norm{X\beta - y}_2^2
\quad \text{s.t.}\quad -u_i\leq \beta_i \qandq \beta_i\leq u_i
\end{align*}
One can either deal with the above directly, or as done in \cite{koh2007interior}, one can 
introducing  a barrier function for the constraints:
\begin{equation}\label{eq:inte_pt}
\min_{\beta,u} \phi_\gamma(u,\beta)\eqdef \gamma \pa{\sum_i u_i + \frac12 \norm{X\beta - y}_2^2} + \sum_i \log(u_i +\beta_i) + \sum_i\log(u_i-\beta_i).
\end{equation}
The idea of interior point methods is to write down the optimality conditions for \eqref{eq:inte_pt} and solve this using Newton's method. That is, one generates sequences $\beta_k,u_k$ where, at each iteration, solve
$$
\begin{pmatrix}
\Delta_\beta \\
\Delta_u
\end{pmatrix} = H^{-1} J
$$
where $H$ is the Hessian of $\phi_\gamma$ and $J$ is the Jacobian of $\phi_\gamma$, evaluated at $\beta_k$, $u_k$. The new point $\beta_{k+1}$, $u_{k+1}$ is updated with the directions $\Delta_\beta$ and $\Delta_u$.


\paragraph{The $\eta$-trick}
One can also write
$$
\sum_{g\in\Gg} \norm{\beta_g}_2 = \min_{\eta\geq 0} \frac12 \sum_g \frac{\norm{\beta_g}^2}{\eta_g} + \frac12 \sum_g \eta_g.
$$
This is the so-called $\eta$-trick and is equivalent to \eqref{eq:noncvx_group} up to a change of variable.

The group-Lasso can then be written as
\begin{align*}
\min_{\eta\geq 0}\hat f_\lambda(\eta)\eqdef \max_{\alpha\in\RR^n}  -\frac{1}{2\lambda} \sum_{g\in\Gg} \eta_g \norm{X_g^\top \alpha}^2 - \dotp{\alpha}{y} +\frac{\lambda}{2} \sum_g \eta_g-\frac12 \norm{\alpha}^2
\end{align*}
with the relationship that the optimal points $\beta,\eta,\alpha$ satisfy
$$
\beta =\frac{1}{\lambda} \eta \odot X^\top \alpha
$$


The basis pursuit problem written as
\begin{align*}
\min_{\eta\geq 0} \hat f_0(\eta)\eqdef  \max_{\alpha\in\RR^n}  -\frac{1}{2} \sum_{g\in\Gg} \eta_g \norm{X_g^\top \alpha}^2 - \dotp{\alpha}{y} +\frac{1}{2} \sum_g \eta_g .
\end{align*}
with the relationship that the optimal points $\beta,\eta,\alpha$ satisfy
$$
\beta = \eta \odot X^\top \alpha.
$$

Both $\hat f_\lambda$ and $\hat f_0$ are differentiable, so we have smooth minimisation problems with positivity constraint. They  can be minimised using any descent algorithm, generating $\eta_k$ as
\begin{itemize}
\item For $\eta=\eta_k$, compute $\nabla \hat f_\lambda(\eta) = \frac{\lambda}{2} - \frac{\lambda}{2} ( \norm{X_g^\top \alpha})_g$ where $\alpha$ satisfies 
$$
(\lambda X \diag(\eta) X^\top + \Id) \alpha = y
$$
\item  Update $\eta_k$ with $\nabla \hat f_\lambda(\eta_k)$ choosing a stepsize to ensure that $\eta_{k+1}\geq 0$.
\end{itemize}
This is somewhat reminiscent of interior point methods, in the sense that at each iteration, we solve a linear system which comes from the optimality conditions of the dual variable, and update with this as a search direction, while still enforcing the ``interior point constraint" that $\eta_{k+1}\geq 0$. This is in essence the approach of \cite{rakotomamonjy2008simplemkl} (although their context is multiple kernel learning and equation are slightly different).

\paragraph{Differences with our  nonconvex splitting scheme}
\begin{itemize}
\item We write down and solve partially the optimality conditions, our linear system is of size no greater than the problem dimension $n$, whereas, in interior points methods, the linear system to solve have dimension  larger than $n$ as one includes Lagrange multipliers.

\item We have no constraints to enforce. In interior point methods and the $\eta$-trick, either the stepsize is restricted by the inequality constraints, or a barrier function needs to be introduced, and it is these inequality constraints which is the difficulty that interior points methods overcome in clever ways (see Chapter 14 of \cite{nocedal2006numerical}). I think this is the reason why nonconvex splitting is a preferable approach and leads to faster practical performance (although  I don't have anything more concrete to say..)
\item Convergence rate?? Unless the solution is strictly in the interior of the constraints, there is in general at best linear convergence for interior point methods? e.g. \cite{monteiro1994local}??

\item The numerical observation is that the $\eta$ trick converges slower than the nonconvex splitting, and generally leads to less sparse outputs.
\end{itemize}


\subsection{Total variation of functions}
Consider
$$
\min_{\beta\in\RR^n} \lambda \norm{D \beta}_{1} + \frac12\norm{X\beta - y}_2^2.
$$
This can be written as
$$
\min_{\beta,v,a\in\RR^n}\frac{ \lambda}{2} \pa{\norm{v}^2 + \norm{u}^2} + \frac12\norm{X\beta - y}_2^2 \qwhereq D \beta = v\odot u
$$
By convex duality, over the variable $u$,
\begin{align*}
&\min_{\beta,v,a\in\RR^n}  \max_{\alpha}\frac{\lambda}{2} \pa{\norm{v}^2 + \norm{u}^2} + \frac12\norm{X\beta - y}_2^2 +\dotp{\alpha}{ D \beta - v\odot u}\\
& = \min_{\beta,v\in\RR^n}  \max_{\alpha}\frac{\lambda}{2} \norm{v}^2 - \frac{1}{2\lambda} \norm{v\odot(D^* \alpha)}^2 + \frac12\norm{X\beta - y}_2^2 +\dotp{\alpha}{ D \beta }\\
&= \min_{\beta,v\in\RR^n} f(\beta,v) \eqdef   \max_{\alpha}\frac{\lambda}{2} \norm{v}^2 - \frac{1}{2\lambda} \norm{v\odot(D^* \alpha)}^2 + \frac12\norm{X\beta - y}_2^2 +\dotp{\alpha}{ D \beta }.
\end{align*}
For each $\beta,v\in\RR^n$, $\alpha$ can be computed as 
$$
\frac{1}{\la} D(v^2 \odot D^* \alpha) = D\beta,
$$
and $\partial_\beta f = X^\top (X\beta - y) + D^* \alpha$, $\partial_t f = \lambda t + \frac{1}{\la} v\odot \abs{D^*\alpha}^2 $.
\todo{differentiability breaks here if this linear system does not have a unique solution, for $f$ to be differentiable, we need $D^*\alpha$ to be unique.}

\subsection{Non-overlapping groups}
The same technique can be applied to the case of non-overlapping group Lasso: consider
\begin{equation}
\min_{\beta\in\RR^n, \hat \beta_g\in\RR^{n_g}}  \sum_{g\in\Gg} \norm{\hat \beta_g} +\frac{1}{2\lambda} \norm{X \beta - y}_2^2 \qwhereq \beta = \sum_{g\in\Gg} S_g^* \hat \beta_g
\end{equation}
where $S_g:\RR^n\to\RR^{n_g}$ is a subsampling operator and $S_g^*$ is its adjoint operator. This is equivalent to
\begin{equation}
\min_{v\in\RR^{\abs{\Gg}}} f(v)\eqdef  \min_{ u_g\in\RR^{n_g}, g\in\Gg}  \frac{1}{2}\norm{v}_2^2 + \frac{1}{2} \sum_{g\in\Gg} \norm{u_g}_2^2 +\frac{1}{2\lambda} \norm{X \sum_{g\in\Gg} S_g^* (v_g u_g) - y}_2^2
\end{equation}
and note that the inner problem can be solved by inverting a linear system.

By convex duality  on the inner problem, another  equivalent formulation is
\begin{align*}
f(v) = &\max_{\alpha\in\RR^m} \min_{ u_g\in\RR^{n_g}}  \frac{1}{2}\norm{v}_2^2 + \frac{1}{2} \sum_{g\in\Gg} \norm{u_g}_2^2 -\frac{1}{2\lambda} \norm{\alpha}_2^2 + \dotp{X \sum_{g\in\Gg} S_g^* (v_g u_g) - y}{\alpha}\\
&=  \max_{\alpha\in\RR^m}  \frac{1}{2}\norm{v}_2^2 -\frac{1}{2} \sum_{g\in\Gg} v_g \norm{S_g  X^\top \alpha}_2^2-\frac{1}{2\lambda} \norm{\alpha}_2^2 - \dotp{y}{\alpha}
\end{align*}
and the inner problem can be solved by inverting a linear system.


\section{Other comments to remind myself only...}

This was how I originally derived the expression for the group l1 norm directly from Theorem 1:
\begin{cor}[group $\ell_1$] Let $R(\beta) = \phi(\beta\odot\beta)$ where $\phi(u) = \sum_{g\in\Gg} \sqrt{ u_g^\top 1_{n_g}}$ which is concave on $\RR_+^n$. The convex conjugate  $\psi (z)= (-\phi)^* (-z)$ satisfies $\psi(z)_i = \frac{1}{4\min_{i\in g} z_i}$ for all $i\in g\in \Gg$.
Therefore
 \begin{equation}\label{eq:eta_l12}
\sum_{g\in\Gg} \norm{\beta_g}_2  = \min_{z\in \RR_+^{\abs{\Gg}}}  \sum_{g\in\Gg} {\norm{\beta_g}_2^2}{z_g}  + \frac14 \sum_{g\in\Gg} \frac{1}{z_g}.
 \end{equation}
\end{cor}
\begin{proof}
This follows by inspecting the KKT conditions:
We can write 
$$
\psi(z) = \max_{u\geq 0}  -\dotp{u}{z} + \phi(u) = - \max_{\lambda\geq 0} \min_u \dotp{u}{z} - \sum_g \sqrt{u_g^\top 1_{n_g}} - \dotp{u}{\lambda}
$$
By inspecting the optimality condition with respect to $u$,
$$
z_i - \lambda_i = \frac{1}{2\sqrt{u_g^\top 1_{n_g}}}, \qquad \forall i\in g
$$
and so, for all $i\in g$, $z_i-\lambda_i = v_g$ for some $v_g \in [0,\min_{i\in g} z_i]$. Moreover,
$$
\dotp{z-\lambda}{u} -\sum_g \sqrt{u_g^\top 1_{n_g}} =- \frac{1}{4}\sum_g \sqrt{u_g^\top 1_{n_g}} = -\sum_{g\in \Gg} \frac{1}{4v_g}
$$
It therefore follows that
\begin{align*}
\psi(z) &= \min_{v\geq 0}\sum_{g\in \Gg} \frac{1}{4v_g}, \qwhereq v_g \in [0,\min_{i\in g} z_i]\\
&= \sum_{g\in \Gg} \frac{1}{4\min_{i\in g} z_i}.
\end{align*}

\end{proof}



 
 
 We can also write $R(w) = \phi(ww^\top) \eqdef \hat \phi(\diag(ww^\top))$ where $\diag$ extracts the diagonal of a matrix and given $z\in\RR^n$, $\hat \phi(z) \eqdef \sum_{g\in\Gg} \sqrt{{z_g^\top 1_{n_g}}}$  where $n_g$ is the size of group $g$. The function $\phi$ is concave and 
\begin{equation}
\psi(D) = (-\phi)^*(-D)= \sup_{Z\in\SS_n^+} -\dotp{Z}{D} + \phi(Z)
\end{equation}
Clearly, $\psi(D)=+\infty$ if $D$ is not diagonal since $\phi(Z)$ ignores all nondiagonal elements of $Z$. Moreover, the optimal $Z$ satisfies $D\in \partial \phi(Z) =\frac12 \diag( \frac{1_{n_g}}{\sqrt{z_g^\top 1_{n_g}}} )$ where $z_g$ is the diagonal of $Z$ corresponding to group $g$  and 
 $\psi(D) = \sum_{g\in\Gg} \frac{1}{4 \min_{i\in g} D_{i,i}}$. 

\subsection{Application: The Benamou-Brenier formulation}
Consider 
$$
\min_{w,\rho; \rho\geq 0} \sum_i c_i \frac{\norm{w_i}^2}{\rho_i} \quad \text{s.t.} \quad D_t \rho + D_x^*(w ) = 0, \; P_0 \rho = \mu,\; P_1 \rho = \nu
$$
where $c_i$ are positive weights. To place an obstacle, we should let $c_i = +\infty$.
Making a change of variable by $u = w/\sqrt{\rho}$ and $v = \sqrt{\rho}$ (where division is in a pointwise sense), we obtain
$$
\min_{u,v} \sum_i c_i\norm{u_i}^2 \quad \text{s.t.} \quad D_t (v\odot v) + D_x^*(u\odot v) = 0, \; P_0 (v\odot v) = \mu,\; P_1 (v\odot v)  = \nu.
$$
This is a convex optimisation problem over the variable $u$ and is equivalent to
\begin{align*}
&\min_v \max_{\alpha}  \min_{u} \frac12  \sum_i c_i\norm{u_i}^2+\dotp{\alpha}{D_t (v\odot v) + D_x^*(u\odot v)} \quad \text{s.t.} \quad P_0 (v\odot v) = \mu,\; P_1 (v\odot v)  = \nu\\
&=\min_v \max_{\alpha}  -\frac12 \sum_i \frac{ v_i^2\norm{(D_x\alpha)_i }_2^2 }{c_i}  +\dotp{\alpha}{D_t (v\odot v) } \quad \text{s.t.} \quad P_0 (v\odot v) = \mu,\; P_1 (v\odot v)  = \nu
\end{align*}
The inner problem requires to solve a weighted Laplace problem
$$
D_x^*(c^{-1}\odot v^2\odot D_x \alpha) =  D_t v^2,
$$
where we write $v^2 \eqdef v\odot v$.
Gradient wrt $v$ is $-\frac{v}{c}\odot \norm{D_x \al}^2 + 2 v\odot(D_t^* \alpha)$.

\paragraph{Dynamic inverse problems}
Consider
\begin{equation}
\min_{\rho,w: \rho\geq 0} \frac12 \sum_i \frac{\norm{w_i}^2}{\rho_i} + \frac{\lambda_1}{2} \sum_i \rho_i + \frac{\lambda_2}{2} \norm{\Phi \rho - y}_2^2 \quad\text{s.t.} \quad D_t\rho + D_x^*(w) = 0
\end{equation}
By convex duality,
\begin{align*}
&\min_{\rho,w: \rho\geq 0} \max_{\alpha} \frac12 \sum_i \frac{\norm{w_i}^2}{\rho_i} + \frac{\lambda_1}{2} \sum_i \rho_i + \frac{\lambda_2}{2} \norm{\Phi \rho - y}_2^2 +\dotp{  D_t\rho + D_x^*(w) }{\alpha} \\
&=\min_{ \rho\geq 0} \max_{\alpha} - \frac12 \sum_i \rho_i\norm{D_x \alpha}^2+ \frac{\lambda_1}{2} \sum_i \rho_i + \frac{\lambda_2}{2} \norm{\Phi \rho - y}_2^2 +\dotp{  D_t\rho }{\alpha}.
\end{align*}
Doing nonconvex splitting
\begin{equation}
\min_v \min_{u} \max_{\alpha} \frac12\norm{u}^2+ \frac{\lambda_1}{2} \norm{v}^2 + \frac{\lambda_2}{2} \norm{\Phi v^2 - y}_2^2+\dotp{  D_t v^2 + D_x^*(u\odot v) }{\alpha} 
\end{equation}
where $v^2 = v\odot v$.
For fixed $v$, the inner problem is a convex problem,  with optimality condition
$$
u + v\odot D_x \alpha = 0
$$
so the problem becomes
\begin{equation}
\min_v \max_{\alpha} -\frac12\norm{v\odot D_x \alpha}^2+ \frac{\lambda_1}{2} \norm{v}^2 + \frac{\lambda_2}{2} \norm{\Phi v^2 - y}_2^2+\dotp{  D_t v^2  }{\alpha} 
\end{equation}




==> sections/smoothproj.tex <==
% !TEX root = ../NonCvxReparam.tex
\newcommand{\fbp}{f_{\mathrm{bp}}}


\section{Projected smooth formulations}
We are often interesting in solving problems of the form
\begin{equation}\label{eq:lasso_gen}
\min_{\beta\in\RR^n}   R(\beta) +\frac{1}{2\lambda} \norm{X\beta - y}_2^2 \tag{$\Pp_\lambda$}
\end{equation}
for some $\lambda>0$ and $X\in\RR^{m\times n}$. In the limit case as $\lambda\to 0$, we consider the constrained problem 
\begin{equation}\label{eq:lasso_gen_bp}
\min_{\beta\in\RR^n}   R(\beta) \quad \text{such that}\quad X\beta = y. \tag{$\Pp_0$}
\end{equation}
For many important regularisers, $R$ admits a quadratic variational form as
\begin{equation}\label{eq:etatrick0}
R(\beta) = \min_{\eta \in\RR^k_+}  \frac{1}{2} \sum_{g\in\Gg} \frac{\norm{\beta_g}_2^2}{\eta_g} +\frac{1}{2} h(\eta).
\end{equation}
where $\Gg$ is a partition on $\ens{1,\ldots, n}$ and $k = \abs{\Gg}$ is the number of groups and $h:\RR^k_+\to [0,\infty)$. An important example is the  group-$\ell_1$ regularisation, where we have $h(\eta) = \sum_i \eta_i$. The case of $\ell_1$, $g= \ens{i}$ for $i=1,\ldots, n$. As we discuss in Section \ref{sec:quad-var},  this formulation is in fact very general and  many of the popular regularisers can be written in this way.


\paragraph{Iterative reweighted least squares}
Due to the $1/\eta_g$ term, one  needs to introduce some regularisation to carry out an alternating minimisation procedure, and one popular approach is to add $\frac{\epsilon}{2}\sum_g \eta_g^{-1}$ which leads to the iterative reweighted least squares (IRLS) algorithm \cite{daubechies2010iteratively} \footnote{Strictly speaking, IRLS deals with the basis pursuit problem where instead of the quadratic loss term, one has the constraint $X\beta = y$. In this work, the case of basis pursuit is discussed in Section \ref{sec:BP}.}, that is, $R$ is replaced by
$$
R_\epsilon(\beta,\eta) = \frac12 \sum_i \frac{\norm{\beta_g}_2^2}{\eta_g} +\frac12 \sum_g \eta_g + \frac{\epsilon}{2}\sum_g \eta_g^{-1},
$$
and we minimise \eqref{eq:lasso_gen} over both $\beta$ and $\eta$.
The $\epsilon$-term can be seen as a barrier to keep $\eta_g$ positive which is  reminiscent of interior point methods. The idea of IRLS is to do  alternating minimisation, where the minimisation with respect to $\beta$ is a least squares problem, and the minimisation with respect to $\eta$ admits a closed form solution.
%\begin{enumerate}
%\item Solve the least squares problem $\beta^{t+1} = \argmin_\beta R_\epsilon(\beta,\eta^t) + \frac12 \norm{X \beta - y}_2^2$.
%\item Decrease $\epsilon$.
%\item Minimise with respect to $\eta$: $\eta^{t+1}_g = \sqrt{\norm{\beta_g}^2_2 +\frac{ \epsilon}{\lambda}}$.
%\end{enumerate}

\paragraph{Reduced problem and first order methods}
Another approach discussed in several works \cite{bach2011optimization,pong2010trace,rakotomamonjy2008simplemkl} is to apply descent methods over $g(\eta) \eqdef \min_\beta R_0(\eta,\beta)+\frac12 \norm{X\beta - y}_2^2$. Although the function over $\eta$ and $\beta$ is discontinuous, the function $g$ over $\eta$ is smooth  and   one can apply first order methods, such as proximal gradient descent to minimise $g$ under positivity constraints.
%Or (as we explain later), one can rewrite the inner optimisation problem over $\beta$ as a maximisation problem and carry out a smooth optimisation problem with positivity constraints 

\paragraph{New approach: Nonconvex reparametrization with variable projection}
In this paper, we make a simple observation that a nonconvex reparametrization  leads to a smooth unconstrained optimisation problem, and rather than doing alternating minimisation, we propose to  solve a bilevel problem using LBFGS.
%
 The outcome is that we retain the simplicity of iterative reweighted least squares without the need for extra regularisation, we benefit from the improvement in problem conditioning by solving a reduced problem, while having a completely smooth unconstrained problem which allows for the use of a wide range of  optimisation  methods, in particular, quasi-Newton methods such as L-BFGS which leasds to  local superlinear convergence properties. In our numerical examples, we show that this is a very versatile idea and can lead to significant computational gains.

%



\begin{prop}\label{prop:grad}
The problem \eqref{eq:lasso_gen} is equivalent to
\begin{align}
\min_{v\in\RR^k}  f(v) &\eqdef  \min_{u\in\RR^n} \frac{1}{2} h(v\odot v) + \frac{1}{2} \norm{u}^2 + \frac{1}{2\lambda} \norm{X(v\odot_\Gg u) - y}_2^2. \label{eq:noncvx}\\
&=\max_{\alpha\in\RR^m}   \frac{1}{2} h(v\odot v) -\frac{\lambda}{2}\norm{\alpha}_2^2 - \frac{1}{2} \norm{v\odot_\Gg(X^\top \alpha)}_2^2  + \dotp{\alpha}{  y}. \label{eq:noncvx2}
\end{align}
where $v\odot_\Gg u = (u_g v_g)_{g\in\Gg}$.
The function $f$  is smooth  and  its  gradient at $v\in\RR^k$ can be written as
\begin{align}
\nabla f(v) &=   v\odot \partial h(v^2) +\frac{1}{\la}\pa{ \dotp{ u_g}{ X_g^\top( X (v\odot_\Gg u) - y )   }}_{g\in\Gg} \label{eq:gradform1}\\
&=  v \odot \partial h(v^2) - v \odot_\Gg  \pa{\norm{X_g^\top \alpha}^2}_{g\in\Gg}   \label{eq:gradform2}
\end{align}
where $u\in \RR^n$ in \eqref{eq:gradform1} satisfies \begin{equation}\label{eq:gradf1}
( \diag(\bar v) X^\top X \diag(\bar v)  +\lambda\Id) u =v\odot_\Gg ( X^\top y).
\end{equation}
where $\bar v$ is defined such that $\bar v \odot u = (v_g u_g)_{g\in\Gg}$ for all $u\in\RR^n$,
and  $\alpha\in \RR^m$ in \eqref{eq:gradform2} satisfies
\begin{equation}\label{eq:gradf2}
(   X \diag(\bar v^2) X^\top + \la \Id ) \alpha = y.
\end{equation}
The minimiser $\beta$ to \eqref{eq:lasso_gen} and the minimiser $v$ to \eqref{eq:noncvx} are related by
$
\beta = v\odot_\Gg u =  v^2\odot_\Gg X^\top \alpha.
$

When $\lambda = 0$, \eqref{eq:lasso_gen_bp} is equivalent to \eqref{eq:noncvx2} with $\lambda = 0$ which is a smooth function with  gradient is  as \eqref{eq:gradform2} with $\alpha$ computed as in \eqref{eq:gradf2}.  Note that the gradient is well defined as $v\odot_\Gg X^\top \al$ is unique  even if there are multiple solutions to \eqref{eq:gradf2}.
\end{prop}


\begin{rem}
Observe that by the equivalence to \eqref{eq:noncvx} follows by letting $v_g= \sqrt{\eta_g}$ and $u_g = \beta_g/\sqrt{\eta_g}$ in \eqref{eq:etatrick0},  The fact that $f$ is smooth simply follows by the fact that the inner minimisation problem has a unique solution.  A detailed proof can be found in Appendix \ref{}. 
\end{rem}
\paragraph{Computation of the gradient}
In general, the complexity of computing $\nabla f(v)$ is $\Oo(sm + r)$ where $r= \min\ens{n^3,m^3}$ if one directly inverts the linear systems.   Note that in both cases, the linear system to invert is symmetric positive semidefinite, and when $s$ and $m$ are both large, one can approximately invert the linear systems by  applying conjugate gradient. Compared to first order methods, so there is in general an increase in per iteration cost of $r$, however, since we can apply higher order methods with a faster order of convergence, we still observe significant gains in practice (see Section \ref{sec:numerics_lasso} for numerical illustrations). 
%Note that typical first order methods for solving \eqref{eq:lasso_gen} require computing the gradient of the smooth part which has complexity $\Oo(mn)$, in  cases where the number of groups $k$ can be much smaller than $n$,  one can obtain a  reduction in per iteration cost by  dealing with \eqref{eq:noncvx}. On the other hand, for the Lasso, we have $k=n$, so there is in general an increase in per iteration cost of $\Oo(\min\pa{m^3, n^3})$, however, since we can apply higher order methods with a faster order of convergence, we still observer significant gains in certain problems (see Section \ref{sec:numerics_lasso} for numerical illustrations).

\paragraph{Non-convexity} Although $f$ is a non-convex function, this non-convexity is only mild in the sense that there are no local minimums: all stationary points are either global minimums or strict local minimums, see Section \ref{sec:gradientprops} for the details. As a result, one can guarantee convergence to a global minimum for many optimisation schemes, such as  gradient descent with random perturbations \cite{lee2017first,jin2017escape} or trust region type methods \cite{pascanu2014saddle}. 

\paragraph{Other loss functions}
In this paper, we focus on the quadratic loss due to its simple form $L_y(\beta)\eqdef \frac12 \norm{X\beta - y}^2$, it is however possible to extend to other convex (and possibly nonsmooth) loss functions other than the quadratic loss: due to the $\norm{u}^2$ term, the inner problem is strongly convex and has a unique solution. So, as explained in the proof of Proposition \ref{prop:grad},  $f$ is still a smooth function, so the framework described here can still be applied provided that $\min_u \frac12 \norm{u}^2 + L_y(v\odot u)$ can be solved efficiently for each $v$. In Section \ref{sec:BP}, we show how to extend to the case of basis pursuit, where we have affine constraints.

\subsection{Relationship to previous works}\label{sec:biblio-etatrick}

\paragraph{The quadratic variational formulation}
Results of the form given in Theorem 1 have been exploited in many early computer vision works, such as  \cite{geiger1991common}  and \cite{geman1992constrained}. Theorem 1 is similar to Theorem 1 in \cite{geman1992constrained} by Geman and Reynolds, although their proof was only for strictly concave differentiable functions and did not explicitly connect to convex conjugates. The  Geman and Reynolds theorem was later explored in more detail in  by Black and Rangarajan in \cite{black1996unification}, where they provided many examples and we refer to this paper for a nice overview of early works exploiting quadratic variational formulations.  Regularizers of the forms given in \eqref{eq:psi-norm} and \eqref{eq:etatwo} were introduced in \cite{micchelli2013regularizers}, and further elaborated on in the monograph \cite{bach2011optimization}. Our results can be seen as an extension of Lemma 1.9 in  \cite{bach2011optimization}, however, their statement was only for sub-quadratic norms, and Proposition 5.1 of \cite{bach2011optimization}, however, their result is concerned with  vector norms. More recently,  notable examples of  \eqref{eq:psi-norm} and \eqref{eq:etatwo} in the literature include the use of  $\ell_1$ formulation  in \cite{daubechies2010iteratively} for the iteratively reweighted least squares algorithm. The nuclear norm versions have been used in \cite{argyriou2008convex} where an alternating minimisation algorithm was introduced, and also in \cite{pong2010trace}.


\paragraph{Variable projection/reduced gradient approaches}
The idea of minimising a reduced problem is classical, we refer in particular to   Chapter 10 of \cite{rockafellar2009variational} for some general theoretical results on reduced gradients, and also Danskin's theorem (although this is restricted to the convex setting) \cite{bertsekas1997nonlinear}.
Our formulation falls directly into the framework of  variable projection \cite{ruhe1980algorithms,golub2003separable},  introduced initially for solving nonlinear least squares problem. Properties and advantages of variable projection have been studied in \cite{ruhe1980algorithms}. Nonsmooth variable projection is studied in \cite{van2016non}, although we are really  in the classical setting of variable projection in this paper. The idea of variable projection is also used  in multiple kernel learning \cite{rakotomamonjy2008simplemkl}, where they formulate MKL as a smooth problem with simplex constraints.

\paragraph{Quasi-Newton approaches for low complexity regularisers}
The main  approaches to quasi-Newton methods for Lasso in the literature include proximal and variable metric approaches \cite{combettes2014variable,becker2019quasi} and directly incorporating the nonsmooth part into the quadratic approximation (via subgradients) \cite{lewis2013nonsmooth}. However, convergence guarantees the latter  are limited, while proximal techniques only guarantee linear convergence under strong convexity. One of the attractions of our formulation is that standard Quasi-Newton schemes for smooth optimisation can be applied. 


\paragraph{Nonconvex formulations}
Although nonconvex formulations for various low complexity regularisers have appeared in the literature, see for instance  \cite{hoff2017lasso} in the case of the $\ell_1$ norm, and \cite{hastie2015matrix} in the case of the nuclear norm, they are typically associated with alternating minimisation algorithms. 




